The Convergence Rate of Accelerated Proximal Gradient Methods with General Inertial Term for Convex Composite Multiobjective Optimization

We study accelerated proximal gradient methods with general stepsizes for convex composite multiobjective optimization, where each objective is a smooth convex term plus a proper closed convex term and the proximal subproblem keeps a separate offset for each objective. For a two-parameter root momentum rule with trajectory-dependent coefficients, we construct a new energy function and establish an energy identity. This yields sharper convergence guarantees: boundedness, weighted square summability of the displacements, a merit-function rate of $o(k^{-2})$, and displacement decay of $o(k^{-1})$ whenever the first parameter converges to a value in $(0,1)$; the second parameter need not converge or have bounded total variation. At the critical value $\alpha=3$, we obtain $u_0(x^N)\le \frac{2\ell R}{N(N+3)},$ together with $O(1/N)$ displacement decay, square summability, and weak Pareto convergence. The remaining little-$o$ question at $\alpha=3$ is reduced to the vanishing of a nonnegative critical energy. For $1<\alpha<3$, we prove the rate $O(N^{-(\alpha-1)})$, and for every $\alpha>0$ we obtain $u_0(x^k)\to0$, $F_i(x^k)\to c_i$, and $\sum_k D_k/k<\infty$. A JOS1 experiment numerically validates the predicted little-$o$ separation and the rate behavior.

==> refs.tex <==
\begin{thebibliography}{99}
\setlength{\itemsep}{0pt}
\setlength{\parskip}{0pt}

\bibitem{tanabe2019proximal}
Tanabe H, Fukuda E H, Yamashita N. Proximal gradient methods for multiobjective optimization and their applications. Computational Optimization and Applications, 2019, 72(2): 339--361. doi:10.1007/s10589-018-0041-3.

\bibitem{tanabe2023accelerated}
Tanabe H, Fukuda E H, Yamashita N. An accelerated proximal gradient method for multiobjective optimization. Computational Optimization and Applications, 2023, 86(2): 421--455. doi:10.1007/s10589-023-00497-w.

\bibitem{tanabe2023convergence}
Tanabe H, Fukuda E H, Yamashita N. Convergence rates analysis of a multiobjective proximal gradient method. Optimization Letters, 2023, 17(2): 333--350. doi:10.1007/s11590-021-01804-2.

\bibitem{tanabe2022root}
Tanabe H, Fukuda E H, Yamashita N. A globally convergent fast iterative shrinkage-thresholding algorithm with a new momentum factor for single and multi-objective convex optimization. arXiv:2205.05262, 2022.

\bibitem{zhang2023}
Zhang J, Yang X. The convergence rate of the accelerated proximal gradient algorithm for multiobjective optimization is faster than $O(1/k^2)$. arXiv:2312.06913, 2023.

\bibitem{beck2009fista}
Beck A, Teboulle M. A fast iterative shrinkage-thresholding algorithm for linear inverse problems. SIAM Journal on Imaging Sciences, 2009, 2(1): 183--202. doi:10.1137/080716542.

\bibitem{sonntag2024fast}
Sonntag K, Peitz S. Fast multiobjective gradient methods with Nesterov acceleration via inertial gradient-like systems. Journal of Optimization Theory and Applications, 2024, 201: 539--582. doi:10.1007/s10957-024-02389-3.

\bibitem{attouch2017subcritical}
Attouch H, Chbani Z, Riahi H. Rate of convergence of the Nesterov accelerated gradient method in the subcritical case $\alpha\le3$. arXiv:1706.05671, 2017.

\bibitem{rockafellar1970convex}
Rockafellar R T. Convex Analysis. Princeton: Princeton University Press, 1970.

\bibitem{jin2001dynamic}
Jin Y, Olhofer M, Sendhoff B. Dynamic weighted aggregation for evolutionary multi-objective optimization: Why does it work and how? In: Proceedings of the 3rd Annual Conference on Genetic and Evolutionary Computation (GECCO'01), 2001: 1042--1049.

\end{thebibliography}

